Machine Learning Approaches to Energy Consumption Forecasting in Households

We consider the problem of power demand forecasting in residential micro-grids. Several approaches using ARMA models, support vector machines, and recurrent neural networks that perform one-step ahead predictions have been proposed in the literature. Here, we extend them to perform multi-step ahead forecasting and we compare their performance. Toward this end, we implement a parallel and efficient training framework, using power demand traces from real deployments to gauge the accuracy of the considered techniques. Our results indicate that machine learning schemes achieve smaller prediction errors in the mean and the variance with respect to ARMA, but there is no clear algorithm of choice among them. Pros and cons of these approaches are discussed and the solution of choice is found to depend on the specific use case requirements. A hybrid approach, that is driven by the prediction interval, the target error, and its uncertainty, is then recommended.

==> ARMA.tex <==
\section{Auto Regressive Moving Average}\label{arma}

==> IEEEtran/README <==

December 27, 2012


IEEEtran is a LaTeX class for authors of the Institute of Electrical and
Electronics Engineers (IEEE) transactions journals and conferences.
The latest version of the IEEEtran package can be found at CTAN:

http://www.ctan.org/tex-archive/macros/latex/contrib/IEEEtran/

as well as within IEEE's site:

http://www.ieee.org/

For latest news, helpful tips, answers to frequently asked questions,
beta releases and other support, visit the IEEEtran home page at my
website:

http://www.michaelshell.org/tex/ieeetran/

V1.8 is a significant update over the 1.7a release. For a full list of
changes, please read the file changelog.txt. The most notable changes
include:


 1) New transmag class option to support the IEEE Transactions on Magnetics
    format. Thanks to Wei Yingkang, Sangmin Suh and Benjamin Gaussens
    for suggestions and beta testing.

 2) The \IEEEcompsoctitleabstractindextext and 
    \IEEEdisplaynotcompsoctitleabstractindextext
    commands have been deprecated in favor of their
    \IEEEtitleabstractindextext and \IEEEdisplaynontitleabstractindextext
    (observe that the "not" has changed to "non") equivalents. This change
    generalizes and decouples them from compsoc mode because the new
    transmag mode also uses them now.

 3) Added new *-forms of \IEEEyesnumber*, \IEEEnonumber*, \IEEEyessubnumber*,
    and \IEEEnosubnumber* (the non-star form of the latter is also new) which
    persist across IEEEeqnarray lines until countermanded. To provide for
    continued subequations across instances of IEEEeqnarrays as well as for
    subequations that follow a main equation (e.g., 14, 14a, 14b ...)
    \IEEEyessubnumber no longer automatically increments the equation number
    on it's first invocation of a subequation group. Invoke both
    \IEEEyesnumber\IEEEyessubnumber together to start a new
    equation/subequation group.
 
 4) Hyperref links now work with IEEEeqnarray equations.
    Thanks to Stefan M. Moser for reporting this problem.

 5) Revised spacing at top of top figures and tables to better
    align with the top main text lines as IEEE does in its journals. 
    Thanks to Dirk Beyer for reporting this issue and beta testing.


Best wishes for all your publication endeavors,

Michael Shell
http://www.michaelshell.org/


********************************** Files **********************************

README                 - This file.

IEEEtran.cls           - The IEEEtran LaTeX class file.

changelog.txt          - The revision history.

IEEEtran_HOWTO.pdf     - The IEEEtran LaTeX class user manual.

bare_conf.tex          - A bare bones starter file for conference papers.

bare_jrnl.tex          - A bare bones starter file for journal papers.

bare_jrnl_compsoc.tex  - A bare bones starter file for Computer Society
                         journal papers.

bare_jrnl_transmag.tex - A bare bones starter file for IEEE Transactions
                         on Magnetics journal papers.

bare_adv.tex           - A bare bones starter file showing advanced
                         techniques such as conditional compilation,
                         hyperlinks, PDF thumbnails, etc. The illustrated
                         format is for a Computer Society journal paper.

***************************************************************************
Legal Notice:
This code is offered as-is without any warranty either expressed or
implied; without even the implied warranty of MERCHANTABILITY or
FITNESS FOR A PARTICULAR PURPOSE! 
User assumes all risk.
In no event shall IEEE or any contributor to this code be liable for
any damages or losses, including, but not limited to, incidental,
consequential, or any other damages, resulting from the use or misuse
of any information contained here.

All comments are the opinions of their respective authors and are not
necessarily endorsed by the IEEE.

This work is distributed under the LaTeX Project Public License (LPPL)
( http://www.latex-project.org/ ) version 1.3, and may be freely used,
distributed and modified. A copy of the LPPL, version 1.3, is included
in the base LaTeX documentation of all distributions of LaTeX released
2003/12/01 or later.
Retain all contribution notices and credits.
** Modified files should be clearly indicated as such, including  **
** renaming them and changing author support contact information. **

File list of work: IEEEtran.cls, IEEEtran_HOWTO.pdf, bare_adv.tex,
                   bare_conf.tex, bare_jrnl.tex, bare_jrnl_compsoc.tex,
                   bare_jrnl_transmag.tex
***************************************************************************


==> LSTM.tex <==
\subsection{Long Short-Term Memory Neural Networks}\label{lstm}
Long Short-Term Memory (LSTM) networks~\cite{lstm} are a particular class of recurrent ANNs in which the neurons in the hidden layers are replaced with the so-called \textit{memory cells} (MC). A MC is a particular structure that allows to store or forget information regarding the past states of the network. This is made possible by structures called \textit{gates}. Gates are composed by the cascade of a neuron with sigmoidal activation function and a pointwise multiplication. 

\fig{fig:lstm_cell} shows the structure of a typical MC. The input gate is a neuron with sigmoidal activation function. Its output determines the fraction of the MC input that is fed to cell state block. Similarly, the forget gate processes the information that is recurrently fed back into the cell state block. The output gate, instead, determines the fraction of the output of the cell state that should be used as output of the MC at each time step. All the internal connections of the MC have unitary weight. Thanks to this architecture, the output of each memory cell depends possibly on the complete past of its states. This make the LSTM ANNs particularly suitable for processing time series with long time dependencies between the various samples.

\begin{figure}
\center
\def\svgwidth{0.7\columnwidth}
\input{./figures/lstm_cell.eps_tex}
\caption{Example of LSTM Memory Cell (MC).\label{fig:lstm_cell}}
\end{figure}

\fig{fig:lstm} shows an example of the LSTM ANNs considered in this work. As for the NAR networks considered in \secref{nar}, we consider the sequence $X_{\tau-n}^{\tau}$ as input of the network. The $n$ time samples are fed as input to the $4$ memory cells. As the current time $\tau$ goes on, the output of the memory cells depends on the current input sequence $X_{\tau-n}^{\tau}$ and on the previous sequences $X_{\tau-n}^{\tau-i},\ i=i,\dots$ as well. As for the NAR case, the output of the hidden layer is then filtered through a linear neuron to provide the network output.

\begin{figure}
\center
\def\svgwidth{0.7\columnwidth}
\input{./figures/lstm.eps_tex}
\caption{Example of LSTM network with $n$ inputs, one hidden layer with $4$ Memory Cells (MC) and $1$ output neuron.\label{fig:lstm}}
\end{figure}


==> NAR.tex <==
\subsection{Nonlinear Autoregressive Neural Networks}\label{nar}

Non linear autoregressive neural networks (NARs) are recurrent ANNs performing regression tasks on time series~\cite{NNs}. A NAR network operates on a time series $X$ by processing, at each time step $\tau$, the subsequence $X_{n}^{\tau}$ (i.e., the last $h$ values of $X$) and the previous NAR's output $\hat{x}_{\tau}$. The parameter $n$ determines how far in the past the network tries to capture the correlation structure of the input data. In order to capture the nonlinear structure of the considered time series, it is required that neurons in the hidden layers have nonlinear activation functions. The output layer, instead, is composed by neurons with linear activation functions in order for the output not to be bounded to any particular dimension. 

\begin{figure}
\center
\def\svgwidth{0.7\columnwidth}
\input{./figures/nar.eps_tex}
\caption{Example of NAR network with $n$ inputs, one hidden layer with $4$ neurons and $1$ output neuron.\label{fig:nar}}
\end{figure}

\fig{fig:nar} shows an example NAR network. This network takes as input the sequence $X_{\tau-n}^{\tau}$ and the output generated by the network during the previous time step. These inputs are processed by a hidden layer composed of four neurons with $\sigma$ activation functions. The output of the hidden layer is then processed by a linear neuron to produce the desired result.


